Conformer: Convolution-augmented Transformer for Speech Recognition

Recently Transformer and Convolution neural network (CNN) based models have shown promising results in Automatic Speech Recognition (ASR), outperforming Recurrent neural networks (RNNs). Transformer models are good at capturing content-based global interactions, while CNNs exploit local features effectively. In this work, we achieve the best of both worlds by studying how to combine convolution neural networks and transformers to model both local and global dependencies of an audio sequence in a parameter-efficient way. To this regard, we propose the convolution-augmented transformer for speech recognition, named Conformer. Conformer significantly outperforms the previous Transformer and CNN based models achieving state-of-the-art accuracies. On the widely used LibriSpeech benchmark, our model achieves WER of 2.1%/4.3% without using a language model and 1.9%/3.9% with an external language model on test/testother. We also observe competitive performance of 2.7%/6.3% with a small model of only 10M parameters.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> LaTeX 2/00_intro.tex <==
\section{Introduction}
End-to-end automatic speech recognition (ASR) systems based on neural networks have seen large improvements in recent years.
Recurrent neural networks (RNNs) have been the de-facto choice for ASR~\cite{chiu2018state, rao2017exploring, Ryan19, tara2020} as they can model the temporal dependencies in the audio sequences effectively \cite{graves2012sequence}. Recently, the Transformer architecture based on self-attention~\cite{vaswani2017attention, zhang2020transformer} has enjoyed widespread adoption for modeling sequences due to its ability to capture long distance interactions and the high training efficiency. Alternatively, convolutions have also been successful for ASR~\cite{li2019jasper, kriman2019quartznet, han2020contextnet, sainath2013deep, abdel2014convolutional}, which capture local context progressively via a local receptive field layer by layer. 


However, models with self-attention or convolutions each has its limitations. While Transformers are good at modeling long-range global context, they are less capable to extract fine-grained local feature patterns. Convolution neural networks (CNNs), on the other hand, exploit local information and are used as the de-facto computational block in vision. They learn shared position-based kernels over a local window which maintain translation equivariance and are able to capture features like edges and shapes. One limitation of using local connectivity is that you need many more layers or parameters to capture global information. To combat this issue, contemporary work ContextNet~\cite{han2020contextnet} adopts the squeeze-and-excitation module~\cite{hu2018squeeze} in each residual block to capture longer context. However, it is still limited in capturing dynamic global context as it only applies a global averaging over the entire sequence.

Recent works have shown that combining convolution and self-attention improves over using them individually~\cite{bello2019attention}. Together, they are able to learn both position-wise local features, and use content-based global interactions. Concurrently, papers like \cite{yang2019convolutional, yu2018qanet} have augmented self-attention with relative position based information that maintains equivariance. Wu et al. \cite{wu2020lite} proposed a multi-branch architecture with splitting the input into two branches: self-attention and convolution; and concatenating their outputs. Their work targeted mobile applications and showed improvements in machine translation tasks.

\begin{figure}[t]
    \includegraphics[width=0.8\columnwidth]{figure/conformer_new.pdf}
    \caption{\textbf{Conformer encoder model architecture.} Conformer comprises of two macaron-like feed-forward layers with half-step residual connections sandwiching the multi-headed self-attention and convolution modules. This is followed by a post layernorm.}
    \label{fig:conformer}
\end{figure}


\label{sec:model:convolution}
\begin{figure*}
    \centering
    \includegraphics[width=0.7\textwidth]{figure/conv_block.pdf}
    \caption{\textbf{Convolution module.} The convolution module contains a pointwise convolution with an expansion factor of 2 projecting the number of channels with a GLU activation layer, followed by a 1-D Depthwise convolution. The 1-D depthwise conv is followed by a Batchnorm and then a swish activation layer.  }
    \label{fig:conv}
\end{figure*}


In this work, we study how to organically combine convolutions with self-attention in ASR models. We hypothesize that both global and local interactions are important for being parameter efficient. To achieve this, we propose a novel combination of self-attention and convolution will achieve the best of both worlds -- self-attention learns the global interaction whilst the convolutions efficiently capture the relative-offset-based local correlations.
%
Inspired by Wu et al. \cite{wu2020lite, lu2019understanding}, we introduce a novel combination of self-attention and convolution, sandwiched between a pair feed forward modules,  as illustrated in Fig~\ref{fig:conformer}.  

Our proposed model, named Conformer, achieves state-of-the-art results on LibriSpeech, outperforming the previous best published Transformer Transducer \cite{zhang2020transformer} by 15\% relative improvement on the testother dataset with an external language model. We present three models based on model parameter limit constraints of 10M , 30M and 118M.
Our 10M model shows an improvement when compared to similar sized contemporary work \cite{han2020contextnet} with 2.7\%/6.3\% on test/testother datasets. 
Our medium 30M parameters-sized model already outperforms  transformer transducer published in  \cite{zhang2020transformer} which uses 139M model parameters.
With the big 118M parameter model, we are able to achieve 2.1\%/4.3\% without using language models and 1.9\%/3.9\% with an external language model.

We further carefully study the effects of the number of attention heads, convolution kernel sizes, activation functions, placement of feed-forward layers, and different strategies of adding convolution modules to a Transformer-based network, and shed light on how each contributes to the accuracy improvements.

==> LaTeX 2/01_model.tex <==
\section{Conformer Encoder}

Our audio encoder first processes the input with a convolution subsampling layer and then with a number of conformer blocks, as illustrated in Figure~\ref{fig:conformer}. The distinctive feature of our model is the use of Conformer blocks in the place of Transformer blocks as in~\cite{zhang2020transformer, karita2019comparative}.


A conformer block is composed of four modules stacked together, i.e, a feed-forward module, a self-attention module, a convolution module, and a second feed-forward module in the end. 
Sections~\ref{sec:model:atten}, \ref{sec:model:convolution}, and \ref{sec:model:ffn} introduce the self-attention,  convolution, and feed-forward modules, respectively. Finally, \ref{sec:model:conformer} describes how these sub blocks are combined.


\subsection{Multi-Headed Self-Attention Module}
\label{sec:model:atten}

We employ multi-headed self-attention (MHSA) while integrating an important technique from Transformer-XL \cite{dai2019transformerxl}, the relative sinusoidal positional encoding scheme. The relative positional encoding allows the self-attention module to generalize better on different input length and the resulting encoder is more robust to the variance of the utterance length. We use pre-norm residual units~\cite{wang-etal-2019-learning-deep, nguyen2019transformers} with dropout which helps training and regularizing deeper models. Figure~\ref{fig:mhsa} below illustrates the multi-headed self-attention block.

\label{sec:model:atten:selfatten}
\begin{figure}[h!]
\includegraphics[width=0.9\columnwidth]{figure/mhsa.pdf}
    \caption{\textbf{Multi-Headed self-attention module.} We use multi-headed self-attention with relative positional embedding in a pre-norm residual unit.} 
    \label{fig:mhsa}
\end{figure}

\subsection{Convolution Module}
Inspired by \cite{wu2020lite}, the convolution module starts with a gating mechanism \cite{dauphin2017language}---a pointwise convolution and a gated linear unit (GLU). This is followed by a single 1-D depthwise convolution layer.
Batchnorm is deployed just after the convolution to aid training deep models. Figure~\ref{fig:conv} illustrates the convolution block.

\subsection{Feed Forward Module}
\label{sec:model:ffn}
The Transformer architecture as proposed in \cite{vaswani2017attention} deploys a feed forward module after the MHSA layer and is composed of two linear transformations and a nonlinear activation in between. A residual connection is added over the feed-forward layers, followed by layer normalization.
This structure is also adopted by Transformer ASR models~\cite{zhang2020transformer, dong2018speech}.

We follow pre-norm residual units~\cite{wang-etal-2019-learning-deep, nguyen2019transformers} and apply layer normalization within the residual unit and on the input before the first linear layer. We also apply Swish activation \cite{ramachandran2017searching} and dropout, which helps regularizing the network. Figure~\ref{fig:ffn} illustrates the Feed Forward (FFN) module.


\begin{figure*}
    \centering
    \includegraphics[width=0.5\textwidth]{figure/ffn.pdf}
    \caption{\textbf{Feed forward module.} The first linear layer uses an expansion factor of 4 and the second linear layer projects it back to the model dimension. We use swish activation and a pre-norm residual units in feed forward module.}
    \label{fig:ffn}
\end{figure*}

\subsection{Conformer Block}
\label{sec:model:conformer}
Our proposed Conformer block contains two Feed Forward modules sandwiching the Multi-Headed Self-Attention module and the Convolution module, as shown in Figure~\ref{fig:conformer}.

This sandwich structure is inspired by Macaron-Net~\cite{lu2019understanding}, which proposes  replacing the original feed-forward layer in the Transformer block into two half-step feed-forward layers, one before the attention layer and one after.  
As in Macron-Net, we employ half-step residual weights in our feed-forward (FFN) modules. The second feed-forward module is followed by a final layernorm layer.
Mathematically, this means, for input $x_{i}$ to a Conformer block $i$, the output $y_{i}$ of the block is:
\begin{equation}
\begin{split}
    \tilde{x_{i}}&= x_{i} + \frac{1}{2}\mathrm{FFN}(x_{i})    \\
    x'_{i}&= \tilde{x_{i}} + \mathrm{MHSA}(\tilde{x_{i}})    \\
    x''_{i}&= x'_{i} + \mathrm{Conv}(x'_{i})    \\
    y_{i}&= \mathrm{Layernorm}(x''_{i} + \frac{1}{2}\mathrm{FFN}(x''_{i}))    \\
\end{split}
\label{model:conformer:equation}
\end{equation}
where FFN refers to the Feed forward module, MHSA refers to the Multi-Head Self-Attention module, and Conv refers to the Convolution module as described in the preceding sections.

Our ablation study discussed in Sec~\ref{ablate_conformer_macaron} compares the Macaron-style half-step FFNs with the vanilla FFN as used in previous works. We find that having two Macaron-net style feed-forward layers with half-step residual connections sandwiching the attention and convolution modules in between provides a significant improvement over having a single feed-forward module in our Conformer architecture.

The combination of convolution and self-attention has been studied before and one can imagine many ways to achieve that. 
Different options of augmenting convolutions with self-attention are studied in Sec~\ref{ablate_conformer_convolution}.
We found that convolution module stacked after the self-attention module works best for speech recognition.

==> LaTeX 2/02_exp.tex <==
\section{Experiments}
\vskip -0.1in
\label{sec:experiment}
\subsection{Data}
We evaluate the proposed model on the LibriSpeech~\cite{panayotov2015librispeech} dataset, which consists of 970 hours of labeled speech and an additional 800M word token text-only corpus for building language model. We extracted 80-channel filterbanks features computed from a 25ms window with a stride of 10ms. We use SpecAugment \cite{park2019specaugment, largespecaugment} with mask parameter ($F=27$), and ten time masks with maximum time-mask ratio ($p_S = 0.05$), where the maximum-size of the time mask is set to $p_S$ times the length of the utterance.

\subsection{Conformer Transducer}

We identify three models, small, medium and large, with 10M, 30M, and 118M params, respectively, by sweeping different combinations of network depth, model dimensions, number of attention heads and choosing the best performing one within model parameter size constraints. We use a single-LSTM-layer decoder in all our models.
Table ~\ref{tab:model_sizes} describes their architecture hyper-parameters. 

For regularization, we apply dropout \cite{JMLR:v15:srivastava14a} in each residual unit of the conformer, i.e, to the output of each module, before it is added to the module input. We use a rate of $P_{drop} = 0.1$. Variational noise \cite{graves2012sequence, jim1996analysis} is introduced to the model as a regularization. A $\ell_2$ regularization with $1e-6$ weight is also added to all the trainable weights in the network. We train the models with the Adam optimizer \cite{kingma2014adam} with $\beta_{1} = 0.9$, $\beta_{2} = 0.98$ and $\epsilon = 10^{-9}$ and a transformer learning rate schedule \cite{vaswani2017attention}, with 10k warm-up steps and peak learning rate $0.05/\sqrt{\bf{d}}$ where $\bf{d}$ is the model dimension in conformer encoder.   

We use a 3-layer LSTM language model (LM) with width 4096 trained on the LibriSpeech langauge model corpus with the LibriSpeech960h transcripts added, tokenized with the 1k WPM built from LibriSpeech 960h.  The LM has word-level perplexity 63.9 on the dev-set transcripts. The LM weight $\lambda$ for shallow fusion is tuned on the dev-set via grid search. All models are implemented with Lingvo toolkit~\cite{lingvo}.

\begin{table}
\begin{centering}
\caption{Model hyper-parameters for Conformer S, M, and L models, found via sweeping different combinations and choosing the best performing models within the parameter limits.}
\label{tab:model_sizes}
\begin{tabular}{@{}l|ccc@{}}
\hline 
\small
\makecell{Model} & \makecell{Conformer\\ (S)} & \makecell{Conformer\\ (M)} & \makecell{Conformer\\ (L)} \\
\hline 
\hline 
{Num Params (M)} & 10.3 & 30.7 & 118.8  \tabularnewline
{Encoder Layers} & 16 & 16 & 17 \tabularnewline
{Encoder Dim} & 144 & 256 & 512  \tabularnewline
{Attention Heads} & 4 & 4 & 8 \tabularnewline
{Conv Kernel Size} & 32 & 32 & 32 \tabularnewline
{Decoder Layers} & 1 & 1 & 1 \tabularnewline
{Decoder Dim} & 320 & 640 & 640 \tabularnewline
\hline
\end{tabular}
\par\end{centering}
\end{table}


\subsection{Results on LibriSpeech}
\begin{table}[h!]
\caption{Comparison of {\netname} with recent published models. Our model shows improvements consistently over various model parameter size constraints. At 10.3M parameters, our model is 0.7\% better on testother when compared to contemporary work, ContextNet(S) \cite{han2020contextnet}. At 30.7M model parameters our model already significantly outperforms the previous published state of the art results of Transformer Transducer \cite{zhang2020transformer} with 139M parameters.}
\label{tab:results:libri_main_results}
  
  %\vskip 0.1in
  \centering
  \small
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    \bfseries Method & \#{\bfseries Params (M)} & \multicolumn{2}{c}{\bfseries WER Without LM} & \multicolumn{2}{c}{\bfseries WER With LM} \\
    \cmidrule(r){3-4} \cmidrule(r){5-6}
     & & \bfseries testclean & \bfseries testother & \bfseries testclean & \bfseries testother \\
    \midrule
    \bfseries Hybrid \\
    \quad Transformer~\cite{wang2019transformer} & - 
    & - & - & 2.26 & 4.85 \\
    \bfseries CTC \\
    \quad QuartzNet ~\cite{kriman2019quartznet} & 19
    &3.90 & 11.28 & 2.69 & 7.25\\
    \bfseries LAS \\
    \quad  Transformer \cite{synnaeve2019endtoend} & 270
    & 2.89 & 6.98 & 2.33 & 5.17 \\
    \quad Transformer \cite{karita2019comparative} & -
    & 2.2 & 5.6 & 2.6 & 5.7 \\
    \quad LSTM & 360 & 2.6 & 6.0 & 2.2 & 5.2 \\
    \bfseries Transducer \\
    \quad Transformer \cite{zhang2020transformer} & 139
    & 2.4 & 5.6 & 2.0 & 4.6 \\
    \quad ContextNet(S) \cite{han2020contextnet} & 10.8
    & 2.9 & 7.0 & 2.3 & 5.5\\
    \quad ContextNet(M) \cite{han2020contextnet} & 31.4
    & 2.4 & 5.4 & \textbf{2.0} & 4.5\\
    \quad ContextNet(L) \cite{han2020contextnet} & 112.7
    & \textbf{2.1} & 4.6 & \textbf{1.9} & 4.1\\
    \midrule
    \bfseries Conformer (Ours)\\
    \quad\netname(S) & 10.3 & \textbf{2.7} & \textbf{6.3} & \textbf{2.1} & \textbf{5.0} \\
    \quad\netname(M) & 30.7 & \textbf{2.3} & \textbf{5.0} & \textbf{2.0} & \textbf{4.3} \\
    \quad\netname(L) & 118.8 & \textbf{2.1} & \textbf{4.3} & \textbf{1.9} & \textbf{3.9} \\
    \bottomrule
  \end{tabular}}
\end{table}

Table~\ref{tab:results:libri_main_results} compares the (WER) result of our model on LibriSpeech test-clean/test-other with a few state-of-the-art models include: ContextNet~\cite{han2020contextnet}, Transformer transducer~\cite{zhang2020transformer}, and QuartzNet~\cite{kriman2019quartznet}.
All our evaluation results round up to 1 digit after decimal point.

Without a language model, the performance of our medium model already achieve competitive results of $2.3$/$5.0$ on test/testother outperforming the best known Transformer, LSTM based model, or a similar sized convolution model. With the language model added, our model achieves the lowest word error rate among all the existing models. This clearly demonstrates the effectiveness of combining Transformer and convolution in a single neural network. 



\subsection{Ablation Studies}

\subsubsection{Conformer Block vs. Transformer Block}
\label{ablate_conformer_transformer}
A Conformer block differs from a Transformer block in a number of ways, in particular, the inclusion of a convolution block and having a pair of FFNs surrounding the block in the Macaron-style. Below we study these effects of these differences by mutating a Conformer block towards a Transformer block, while keeping the total number of parameters unchanged. Table~\ref{tab:ablation_model} shows the impact of each change to the Conformer block.
%
Among all differences, convolution sub-block is the most important feature, while having a Macaron-style FFN pair is also more effective than a single FFN of the same number of parameters.
Using swish activations led to faster convergence in the Conformer models.
\begin{table}[h]
% \begin{centering}
\caption{\textbf{Disentangling Conformer.}
Starting from a Conformer block, we remove its features and move towards a vanilla Transformer block: (1) replacing SWISH with ReLU; (2) removing the convolution sub-block; (3) replacing the Macaron-style FFN pairs with a single FFN; (4) replacing self-attention with relative positional embedding~\cite{dai2019transformerxl} with a vanilla self-attention layer~\cite{vaswani2017attention}.
All ablation study results are evaluated without the external LM.}
\label{tab:ablation_model}
\begin{tabular}{@{}l|cccc@{}}
\hline 
\makecell{Model\\ Architecture} & \makecell{dev\\ clean} & \makecell{dev\\ other} & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
Conformer Model & 1.9 & 4.4 & 2.1 & 4.3 \tabularnewline
\enskip -- SWISH + ReLU & 1.9 & 4.4 & 2.0 & 4.5 \tabularnewline
\enskip\enskip-- \textbf{Convolution Block} & 2.1 & 4.8 & 2.1 & 4.9 \tabularnewline
\enskip\enskip\enskip-- Macaron FFN & 2.1 & 5.1 & 2.1 & 5.0 \tabularnewline
\enskip\enskip\enskip\enskip-- {Relative Pos. Emb.} & 2.3 & 5.8 & 2.4 & 5.6 \tabularnewline
\hline 
\end{tabular}

\vskip -0.2in
\end{table}

\subsubsection{Combinations of Convolution and Transformer Modules}
\label{ablate_conformer_convolution}
We study the effects of various different ways of combining the multi-headed self-attention (MHSA) module with the convolution module. First, we try replacing the depthwise convolution in the convolution module with a lightweight convolution \cite{wu2019pay}, see a significant drop in the performance  especially on the dev-other dataset. Second, we study placing the convolution module before the MHSA module in our Conformer model and find that it degrades the results by 0.1 on dev-other. 
Another possible way of the architecture is to split the input into parallel branches of multi-headed self attention module and a convolution module with their output concatenated as suggested in \cite{wu2020lite}. We found that this worsens the performance when compared to our proposed architecture.

These results in Table~\ref{tab:sa_conv_order} suggest the advantage of placing the convolution module after the self-attention module in the Conformer block.

\begin{table}[h]
% \begin{centering}

\caption{\textbf{Ablation study of Conformer Attention Convolution Blocks.} Varying the combination of the convolution block with the multi-headed self attention: (1) Conformer architecture; (2) Using Lightweight convolutions instead of depthwise convolution in the convolution block in Conformer; (3) Convolution before multi-headed self attention; (4) Convolution and MHSA in parallel with their output concatenated~\cite{wu2020lite}.
}
\label{tab:sa_conv_order}
\begin{tabular}{@{}l|cc@{}}
\hline 
\makecell{Model Architecture} & \makecell{dev\\ clean} & \makecell{dev\\ other} \\
\hline 
\hline 
Conformer & 1.9 & 4.4 \tabularnewline
{-- Depthwise conv + Lightweight convolution}  & 2.0 & 4.8 \tabularnewline
Convolution block before MHSA  & 1.9 & 4.5  \tabularnewline
Parallel MHSA and Convolution & 2.0 & 4.9 \tabularnewline
\hline 
\end{tabular}
\vskip -0.2in
\end{table}


\subsubsection{Macaron Feed Forward Modules}
\label{ablate_conformer_macaron}
Instead of a single feed-forward module (FFN) post the attention blocks as in the Transformer models, the Conformer block has a pair of macaron-like Feed forward modules sandwiching the self-attention and convolution modules. Further, the Conformer feed forward modules are used with half-step residuals.
Table~\ref{tab:ablation_macaron} shows the impact of changing the Conformer block to use a single FFN or full-step residuals.
%
\begin{table}[h]
\begin{centering}
\caption{\textbf{Ablation study of Macaron-net Feed Forward modules.}
Ablating the differences between the Conformer feed forward module with that of a single FFN used in Transformer models: (1) Conformer; (2) Conformer with full-step residuals in Feed forward modules; (3) replacing the Macaron-style FFN pair with a single FFN.
}
\label{tab:ablation_macaron}
\begin{tabular}{l|cccc}
\hline 
\makecell{Model\\ Architecture} & \makecell{dev\\ clean} & \makecell{dev\\ other} & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
Conformer & 1.9 & 4.4 & 2.1 & 4.3 \tabularnewline
Single FFN & 1.9 & 4.5 & 2.1 & 4.5 \tabularnewline
Full step residuals & 1.9 & 4.5 & 2.1 & 4.5 \tabularnewline
\hline 
\end{tabular}
\par\end{centering}

\end{table}

\subsubsection{Number of Attention Heads}

In self-attention, each attention head learns to focus on different parts of the input, making it possible to improve predictions beyond the simple weighted average. We perform experiments to study the effect of varying the number of attention heads from $4$ to $32$ in our large model, using the same number of heads in all layers. We find that increasing attention heads up to $16$ improves the accuracy, especially over the devother datasets, as shown in Table~\ref{tab:atten_heads}.

\begin{table}[h]
\begin{centering}
\caption{Ablation study on the attention heads in multi-headed self attention.}
\label{tab:atten_heads}
\vskip -0.1in
\begin{tabular}{@{}cc|cccc@{}}
\hline 
\makecell{Attention\\ Heads} & \makecell{Dim per\\ Head} & \makecell{dev\\ clean} & \makecell{dev\\ other} & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
4 & 128 & 1.9 & 4.6 & 2.0 & 4.5 \tabularnewline
8 & 64 & 1.9 & 4.4 & 2.1 & 4.3 \tabularnewline
16 & 32 & 2.0 & 4.3 & 2.2 & 4.4 \tabularnewline
32 & 16 & 1.9 & 4.4 & 2.1 & 4.5 \tabularnewline
\hline
\end{tabular}
\par\end{centering}
\vskip -0.2in
\end{table}

\subsubsection{Convolution Kernel Sizes}
To study the effect of kernel sizes in the depthwise convolution, we sweep the kernel size in $\{3, 7, 17, 32, 65\}$ of the large model, using the same kernel size for all layers. We find that the performance improves with larger kernel sizes till kernel sizes $17$ and $32$ but worsens in the case of kernel size $65$, as show in Table~\ref{tab:kernel_sizes}. On comparing the second decimal in dev WER, we find kernel size 32 to perform better than rest. 

\begin{table}[h]
\begin{centering}
\caption{Ablation study on depthwise convolution kernel sizes.}
\label{tab:kernel_sizes}
\vskip -0.1in
\begin{tabular}{@{}c|cccc@{}}
\hline 
\makecell{Kernel\\ size}  & \makecell{dev\\ clean} & \makecell{dev\\ other} & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
3 & 1.88 & 4.41 & 1.99 & 4.39 \tabularnewline
7 & 1.88 & 4.30 & 2.02 & 4.44 \tabularnewline
17 & 1.87 & 4.31 & 2.04 & 4.38 \tabularnewline
32 & 1.83 & 4.30 & 2.03 & 4.29 \tabularnewline
65 & 1.89 & 4.47 & 1.98 & 4.46 \tabularnewline
\hline
\end{tabular}
\par\end{centering}
\vskip -0.2in
\end{table}

==> LaTeX 2/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> LaTeX 2/LaTeX/00_intro.tex <==
\section{Introduction}

Convolution Neural Network (CNN) based models for speech recognition is attracting an increasing amount of attention~\cite{zhang2017very,zeghidour2018fully,li2019jasper,kriman2019quartznet}. Among them, the Jasper model~\cite{li2019jasper} is the first CNN based model that achieves close to the state-of-the-art word error rate (WER) 2.95\%  on LibriSpeech test-clean \cite{panayotov2015librispeech} with an external neural language model. The main feature behind this model is a deep convolution based encoder with stacked layers of 1D convolutions and skip connections. Various separable convolutions have been utilized to increase the speed of the model\cite{hannun2019sequence,kriman2019quartznet} and improve the WER.

Nevertheless, the WER achieved by the best CNN model~\cite{kriman2019quartznet} is still significantly higher than the WER from the state-of-the-art transformer-transducer based models~\cite{wang2019transformer}. In addition, a CNN model relies on very deep convolutions to achieve high accuracy, imposing a large number of parameters and flops. This makes it prohibitive to deploy a CNN model to the mobile platform. 

In this paper, we address both the accuracy and the computation issues of a CNN model. We propose a new end-to-end CNN architecture for speech recognition that achieves the state-of-the-art WER of 1.8\%/4.6\% on LibriSpeech test-clean/test-other, out performing existing transformer and LSTM based models\cite{zhang2020transformer, wang2019transformer, zeyer2019comparison, karita2019comparative, park2019specaugment}. In addition, our model has significantly smaller number of parameters compared with existing CNN based models\cite{li2019jasper, kriman2019quartznet}.

To improve the accuracy of the model, we redesign the convolutional encoder to blend the utterance level information with the local acoustic information. A traditional CNN based encoder can only extract local information; it is even shown in \cite{luo2016understanding} that the effective receptive field of a CNN encoder in practice is significantly smaller than its theoretic estimation. To address this, we incorporate the squeeze-and-excitation layer \cite{hu2018squeeze} into our CNN encoder. Such a layer squeezes a sequence of feature vectors which encode local information of an audio into a single global context vector, broadcast this context back to each local feature vector, and blend the two via depthwise convolution. This technique guarantees that each convolutional layer has access to the global information in addition to the local features. Empirically, we observe that this squeeze-and-excitation technique introduces the most reduction on the WER, 2\% \zhengdong{confirm} reduction on the WER on the LibriSpeech test-clean.

In addition, we also propose other design choices of the network architecture, such as replacing the CTC loss by the RNN-T loss\cite{graves2012sequence} and using the swiss-activation function\cite{ramachandran2017searching}. Each technique contributes a slight gain; they sum up and help the model reaching the state-of-the-art WER.

To address the computation cost of a CNN model, we introduce a progressive downsampling scheme on the input utterance for more aggressive downsampling. This allow us to reduce the filter size of all the convolution layers to five without significantly reducing the effective receptive field of the entire encoder. As a benefit, we reduce the length of the encoded sequence by as large as $8\times$ while maintaining the model accuracy.

Inspired by the recent works on network scaling~\cite{tan2019efficientnet}, we also allow our net to scale with the number of channels of a convolution filter, enabling us to scale up the network for lower WER at the cost of increased computation, or to significantly reduce the computation while maintaining good WER.

In summary, the main contributions of this paper are:
\begin{itemize}
    \item A CNN encoder architecture with global context that outperforms existing CNN and transformer based models in accuracy,
    \item A progressive downsampling and model scaling scheme to achieve the best accuracy and computation trade-off.
\end{itemize}



==> LaTeX 2/LaTeX/01_model.tex <==
\section{Model}
This section introduces the architecture details of our network. Section~\ref{sec:model:transducer} discusses the high-level design of the network. Then Section~\ref{sec:model:encoder} introduces our convolutional encoder, the most important contribution of this paper. Later Section~\ref{sec:model:encoder_efficiency} discusses how we progressively reduce the temporal length of the input utterance in the network to reduce the computation while maintaining the accuracy. This section concludes with the discussion on model scaling. 

\subsection{End-to-end network: CNN-RNN-Transducer}
\label{sec:model:transducer}
Our network design is based on the RNN-Transducer framework \cite{graves2012sequence, rao2017exploring, he2017streaming}. The network contains three components: audio encoder on the input utterance, label encoder on the input label and a joint network to combine the two and decode. 

We directly use the label encoder and the joint network from \cite{zhang2020transformer}, but propose a new CNN based audio encoder. 

\subsection{Encoder design}
\label{sec:model:encoder}
Let the input sequence be $x^0=(x_1, \ldots, x_T)$ where $T$ is the temporal length of the sequence and $x_i \in\mathbb{R}^N$ is the $N$ dimensional features of each audio frame. The audio encoder operates on $x^0$ and outputs a sequence of encoded features $y=(y_1, \ldots, y_{T'})$ where $y_j\in\mathbb{R}^{N'}$ and $T'$ is the encoded length. Note that here $T'\ne T$ because the audio encoder reduces the length of sequence. To make it formal, let $\mathrm{AudioEncode}(\cdot)$ be the encoding function, we have
\begin{equation}
    (y_1, \ldots, y_{T'}) = \mathrm{AudioEncode}(x_1, \ldots, x_T).
\end{equation}

$y=(y_1, \ldots, y_{T'})$ will be the input to the RNN-T decoder.

We design the $\mathrm{AudioEncode}(\cdot)$ function via stacking multiple blocks of convolutions. Let $\mathrm{C}_k$ represent the $k$-th block of convolution, and let $x^k = \mathrm{C}_{k}(x^{k-1})$. We have
\begin{equation}
\begin{split}
    y = \mathrm{AudioEncode}(x) = \mathrm{C}_K\left(\mathrm{C}_{K-1}\left(\ldots \mathrm{C}_{1}(x)\right)\right)
\end{split}
\end{equation}

Each $\mathrm{C}(\cdot)$ includes five layers of convolution operations, each followed by batch normalization~\cite{goodfellow2016deep} and an activation function. It also contains the skip connection~\cite{he2016deep} as well as the squeeze-and-excitation component~\cite{hu2018squeeze}. Let $m$ represents the number of convolution layers of a block. Let $\mathrm{Conv}$ represent the 1D convolution. Let $\mathrm{SE}$ represent the squeeze-and-excitation module. Under this notation, we have

\begin{equation}
\begin{split}
&\mathrm{C}(x) = \mathrm{SE}\left(f^{m-1}\left(f'(x)\right)\right) + x,\\
&f(x)=\mathrm{Act}(\mathrm{BN}(\mathrm{Conv}(x)))
\end{split}
\end{equation} where $f^m$ means stacking $m$ layers of the function $f(\cdot)$ on the input. Inside each block, the first layer $f'$ can be different from the rest $m-1$ layers $f$ in the number of input and output convolution channels as well as the convolution stride. In addition, $\mathrm{Act}$ represents the activation function, and we've tried both ReLU and swish function~\cite{ramachandran2017searching}. For reader's convenience, we repeat the definition of the swish function here:
\begin{equation}
f(x)=x\cdot \sigma(\beta x)=\frac{x}{1+\exp{\left(-\beta x\right)}},
\end{equation}
where $\beta$ is a trainable parameter. We've observed that the swish function works slightly better than ReLU. Figure~\ref{fig:conv_block} illustrates the block.

\begin{figure}
    \centering
    \includegraphics[width=0.3\columnwidth]{LaTeX/figure/skip.pdf}
    \caption{A convolution block $C_i$ contains a number of convolutions, each followed by squeeze-and-excitation, batch normalization and activation. Skip connection is applied on the output of the final convolution layer.}
    \label{fig:conv_block}
\end{figure}

The Squeeze-and-excitation~\cite{hu2018squeeze} function $\mathrm{SE}(\cdot)$ performs global average pooling on the input $x$ and transforms it into a global channelwise weight $\theta(x)$ and element wise multiply each frame by this weight. We adopt the idea to the 1D case, to be precise,
\begin{equation}
\begin{split}
    \bar{x}&=\frac{1}{T} \sum_{t} x_t\\
    \theta(x)&=\mathrm{Sigmoid}(W_2(\mathrm{Act}(W_1\bar{x} + b_1)) + b_2) \\
    \mathrm{SE}(x)&=\theta(x)\circ x \\
\end{split}
\end{equation}
where $\circ$ means element-wise multiplication. If $x\in\mathbb{R}^d$, we have $W_1\in\mathbb{R}^{d\times d/8}$, and $W_2\in\mathbb{R}^{d/8 \times d}$. Note that $\mathrm{Sigmoid}(\cdot)$ maps its input to $(0, 1)$.

Figure~\ref{fig:squeeze_and_excitation} illustrates the squeeze-and-excitation function.
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{LaTeX/figure/SqueezeAndExcitation.pdf}
    \caption{1D Squeeze-and-excitation module. The input first goes through a convolution layer followed by batch normalization and activation. Then average pooling is applied to condense the conv result into a 1D vector, which is then processed by a bottleneck structure formed by two fully connected (FC) layers with activation functions. The output goes through a Sigmoid function to be mapped to $(0, 1)$, and then tiled and applied on the conv output using pointwise multiplications.}
    \label{fig:squeeze_and_excitation}
\end{figure*}

In our final design, the network has $17$ convolution blocks $C_0, \ldots, C_{16}$. Except $C_0$ and $C_{16}$ which only have one layer of convolution each, all the other convolution blocks have $5$ layers of convolution.

\subsection{Encoder efficiency}
\label{sec:model:encoder_efficiency}
\subsubsection{Progressive downsampling} We use a convolution layer of stride two to reduce the temporal length of the signal by half. In contrast to the previous CNN models that only downsample the input signal at the first layer only, we progressively apply downsampling at three different convolution blocks layers of the network, leading to in a total reduction factor of eight on the input signal. See Figure~\ref{fig:downsampling} for an illustration. This enables significant computation reduction since the computation cost of 1D convolution scales linearly with respect to the temporal length of the input signal. This avoids loss of information at an early stage. In addition, we include a few blocks of convolutions between two consecutive downsampling layers, allocating enough network capacity to extract rich information at a scale. As a result of this careful design, we observe no loss of accuracy when we put the encoder to the RNN-T framework. Section~\ref{sec:experiments} will validate this in experiments.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{LaTeX/figure/Downsample.pdf}
    \caption{The encoder progressive downsamples the input utterance.}
    \label{fig:downsampling}
\end{figure}

\subsubsection{Small filter size} One of the claim from previous CNN works \cite{li2019jasper,kriman2019quartznet} is that larger filter size of the convolution layers benefit the encoder. In contrary, we set the filter size of every single convolution layer in our net to as small as five, and we observe significant improvement on the WER on LibriSpeech test clean. We suspect that the cause of this conter intuitive phenomenon is the effecitve receptive field of an encoder output node; when an output node covers too long segment of the input audio, the model overfits.

To analyze this more, we follow a previous work~\cite{luo2016understanding} and plot the normalized effective receptive field of our model compared against Jasper and QuartzNet in Figure~\ref{fig:yy} before training. We choose $4\sigma$ as the effective receptive field, and observe that the effective receptive field of our model is the smallest among all. Nevertheless, each encoder output covers $2-3$ seconds of audio, which is long enough to contain the pronunciation of a few words. This empirically demonstrates that our choice of small filter size reduces the risk of overfiting; nevertheless the receptive field is big enough to extract rich information from a long enough sequence of local neighboring audio.

\subsection{Model scaling}
Except for the final convolution layer, we allow the number of input channels and the number of output channels of our model to scale linearly with respect to a hyper parameter $\alpha$. Tuning $\alpha$ linearly affects the number of parameters as well as the flops. Due to the finding about the filter size in the previous section, we do not scale the filter size. This is different from EfficientNet which scales more than one design factors together.

Table \ref{tab:xx} summarizes the architecture details of our network. 

\begin{table}[!tb]
    \centering
    \begin{tabular}{ccccc}
        \hline
         Block ID & \makecell{\# Conv \\ Layers} & \makecell{\#Output \\channels} & \makecell{Filter \\ size} & other \\ \hline\hline
         $C_0$ & 1 & 256 & 5 & No residual \\ \hline
         $C_1$-$C_{10}$ & 5 & 256 & 5 & stride of $C_4, C_7$ is $2$\\ \hline
         $C_{11}$-$C_{29}$ & 5 & 512 & 5 & stride of $C_{11}$ is $2$ \\ \hline
         $C_{30}$ & 1 & 640 & 5 & dilation is $2$\\ \hline
    \end{tabular}
    \caption{Configuration of the network}
    \label{tab:table}
\end{table}


% \section{Relationship with the previous works}

% CNN models in speech
% Our work is inspired many previous work on using the CNN 

% ASR models

% CNN models in vision(weihan)

% \paragraph{CNN models in speech}

% Group 2: 


==> LaTeX 2/LaTeX/02_exp.tex <==
\section{Experiment}  
We conduct experiments on the Librispeech \cite{panayotov2015librispeech} dataset which consists of 970 hours of labeled speech and an additional text only corpus for language model training. We extracted 80 dimensional filterbanks features computed using a 25ms window with a stride of 10ms. 
We optimize the network using Adam\cite{adam} and a peak learning rate of $1e-3$. In the first $2000$ steps, the learning rate has a ramp up from $1e-5$ gradually improving to $1e-3$. Variational noise is introduced to the decoder as a regularization. An $\ell_2$ regularization is also incorporated to all the trainable weights in the network. To further improve the accuracy and the generalizability of the network, we employed the SpecAug\cite{park2019specaugment} technique which randomly masked out frequencies of the input utterance for data augmentation. 

\begin{figure}
\begin{centering}
\includegraphics[width=1\columnwidth]{figure/plot_1}
\par\end{centering}
\caption{LibRispeech Testother WER v.s. Model parameters}
\end{figure}

\subsection{Result on LibriSpeech}
Table \ref{tab:libri_speech_main} showed the result of our model on LibriSpeech test-clean/test-other against a few state-of-the-art methods include: transformer transducer, Jasper, QuartzNet and XXX.

Without language model, the performance of our model already surpassed the best known CNN model even with external language model. With the language model added, our model achieves the lowest word error rate among all the existing models. This clearly demonstrated the effectiveness of our model.

\begin{table}
\begin{centering}
\begin{tabular}{c|c|cc|cc}
\hline 
\multirow{2}{*}[-0.5em]{Model} & \multirow{2}{*}[-0.5em]{\#Params(M)} & \multicolumn{2}{c|}{Without LM} & \multicolumn{2}{c}{With LM}\\ \cline{3-6}
& & \makecell{test\\ clean} & \makecell{test\\ other} & \makecell{test \\clean} & \makecell{test \\ other}\\
\hline 
\hline 
QuartzNet~\cite{kriman2019quartznet}& 19 &3.90 & 11.28 & 2.69 & 7.25\tabularnewline
Hybrid~\cite{wang2019transformer}& - & - & - & 2.26 & 4.85\tabularnewline
Transformer~\cite{zhang2020transformer} & 139 & 2.4 & 5.6 & 2.0 & 4.6\tabularnewline
Ours & 30 & \textbf{2.4} & \textbf{5.4} &  & \tabularnewline
Ours & 46 & \textbf{2.3} & \textbf{5.0} &  & \tabularnewline
Ours & 112 & \textbf{2.1} & \textbf{4.6} & \textbf{2.0} & \textbf{4.1}
\\\hline
\hline 
\end{tabular}
\par\end{centering}
\caption{Comparison of our model against other existing models. Our model achieves superior performance both with and without language models.}
\label{tab:libri_speech_main}
\end{table}

% Table 1: With SE, without SE, SE with window size (a few?)

\subsection{Effect of context size}
To validate the effectiveness of adding global context in the CNN model for speech, we performed an ablation study on how the squeeze-and-excitation module affects the WER on LibriSpeech test-clean/test-other. The original model with all squeeze-and-excitation modules removed serves as the baseline to compare with the original model. 
Note that the squeeze-and-excitation module uses the whole utterance as the context; it has the maximal temporal length of context. This motivates us to study how the temporal length of the context impacts the model performance. To reduce the context to a window smaller than the whole utterance, we replace the global average pooling operator of the squeeze-and-excitation module by a convolutional averaging operator with a kernel size that corresponds to the context window; we apply the same fully connected layers on each context vector, and impose it on the feature of each time step. In this study, we tried window size of $100$ and $200$. 

Table~\ref{tab:context_size} illustrated the result.
% Performed on top of a standard model
% Table 2

\begin{table}
\begin{centering}
\begin{tabular}{c|cc}
\hline 
Context & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
None & ? & ? \tabularnewline
256 & ? & ? \tabularnewline
512 & 2.4 & 5.2\tabularnewline
1024 & 2.3 & 5.1\tabularnewline
global & \textbf{2.3} & \textbf{4.9}\\\hline
\hline 
\end{tabular}
\par\end{centering}
\caption{Ablation study on the temporal length of the context. }
\label{tab:libri_speech_main}
\end{table}


\subsection{Depth, width, filter size and downsampling}
\textit{Depth\ \ } We can increase the model capacity by adding extra convolutional blocks that maintains the number of channels of the encoded features. This also introduces additional computations. We perform a sweeping on the number of extra convolutional layers of the baseline model, and summary the WERs on LibriSpeech test-clean/test-other in Table \ref{tab:ablation_depth}. From the table, we can clearly see the reduction on WER due to the extra capacity of the network, until when the number of layers reach $XX$ and the model saturates.
\begin{table}
\begin{centering}
\begin{tabular}{c|cc}
\hline 
\# Extra Layers & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
0 & ? & ? \tabularnewline
15 & ? & ? \tabularnewline
512 & ? & ?\tabularnewline
1024 & ? & ?\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Ablation study on the depth of the network.}
\label{tab:ablation_depth}
\end{table}


\vspace{0.1in}
\noindent \textit{Width\ \ }

\begin{table}
\begin{centering}
\begin{tabular}{c|ccc}
\hline 
$\alpha$ & \#Params(M) & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
1.25 & 46 & 2.3 & 4.9 \tabularnewline
1.5 & 46 & 2.2 & 4.8 \tabularnewline
1.75 & 87 & 2.2 & 4.7\tabularnewline
2 & 112 & 2.2 & 4.6\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Ablation study on the width of the network.}
\label{tab:ablation_depth}
\end{table}

We also scale the width of the network (i.e., the number of channels) and sees how it impacts the model performance. Specifically, we take the baseline model and scale up the output number of channels of all the convolutional kernels by $\alpha, \alpha > 1$. \zhengdong{What would be the observation?}

\vspace{0.1in}
\noindent
\textit{Downsampling and filter size\ \ }
Table \ref{tab:ablation_downsampling} summarizes the flops and WER on LibriSpeech with and without progressive downsampling. For the reference model with no progressive downsampling, we use the same CNN architectur from the QuartzNet, whose filter size ranges from $11$ to $70$\zhengdong{Confirm}. For the model with progressive downsampling, we sweep the filter size in $\{5, 11, 21\}$. Table \ref{tab:ablation_downsampling} suggests that progressive downsampling introduces significant saving in the number of flops. Moreover, it actually benefits the accuracy of the model slightly. In addition, with progressive downsampling, increasing the filter size hurts the model. This suggests model overfitting.

To qualitatively understand this phenomenon, we plot the initial receptive field of each of the models at each encoder output time step using the technique from \cite{luo2016understanding}. Figure ~\ref{fig:effective_receptive_field} plots the result. Clearly we can see that an encoder output of the QuartzNet architecture effecitvely covers the entire utterance spanning tens of seconds. Our network is much more modest, but still covers a few seconds of an audio sequence to extract rich enough information.

\subsection{Large scale dataset}
Finally, we show that the proposed architecture is also effective on large scale datasets. We use a experimental setup similar to \cite{Chiu19longform}, where the training set has 200K hours of public Youtube videos with semi-supervised transcripts generated by the approach in \cite{hank}. We evaluate on two test sets: \textit{Yt-long } of 87 videos with a total of 24.12 hours and \textit{Yt-short} of 119 videos with a total duration of 24.12 hours. Both sets come with diverse and challenging acoustic environments.

% Preview source code for paragraph 0

\begin{table}
\begin{centering}
\begin{tabular}{cccc}
\hline 
Model & \#Params (M) & YT-short & YT-long\tabularnewline
\hline 
\hline 
LSTM & 192 & 9.1 & 14.8\tabularnewline
CNN & 112 & 9.0 & 14.6\tabularnewline
CNN & 178 & 8.4 & 14.4\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Comparison with previous best results on Youtube test sets}

\end{table}




==> LaTeX 2/LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> LaTeX/00_intro.tex <==
\section{Introduction}

Convolution Neural Network (CNN) based models for speech recognition is attracting an increasing amount of attention~\cite{zhang2017very,zeghidour2018fully,li2019jasper,kriman2019quartznet}. Among them, the Jasper model~\cite{li2019jasper} is the first CNN based model that achieves close to the state-of-the-art word error rate (WER) 2.95\%  on LibriSpeech test-clean \cite{panayotov2015librispeech} with an external neural language model. The main feature behind this model is a deep convolution based encoder with stacked layers of 1D convolutions and skip connections. Various separable convolutions have been utilized to increase the speed of the model\cite{hannun2019sequence,kriman2019quartznet} and improve the WER.

Nevertheless, the WER achieved by the best CNN model~\cite{kriman2019quartznet} is still significantly higher than the WER from the state-of-the-art transformer-transducer based models~\cite{wang2019transformer}. In addition, a CNN model relies on very deep convolutions to achieve high accuracy, imposing a large number of parameters and flops. This makes it prohibitive to deploy a CNN model to the mobile platform. 

In this paper, we address both the accuracy and the computation issues of a CNN model. We propose a new end-to-end CNN architecture for speech recognition that achieves the state-of-the-art WER of 1.8\%/4.6\% on LibriSpeech test-clean/test-other, out performing existing transformer and LSTM based models\cite{zhang2020transformer, wang2019transformer, zeyer2019comparison, karita2019comparative, park2019specaugment}. In addition, our model has significantly smaller number of parameters compared with existing CNN based models\cite{li2019jasper, kriman2019quartznet}.

To improve the accuracy of the model, we redesign the convolutional encoder to blend the utterance level information with the local acoustic information. A traditional CNN based encoder can only extract local information; it is even shown in \cite{luo2016understanding} that the effective receptive field of a CNN encoder in practice is significantly smaller than its theoretic estimation. To address this, we incorporate the squeeze-and-excitation layer \cite{hu2018squeeze} into our CNN encoder. Such a layer squeezes a sequence of feature vectors which encode local information of an audio into a single global context vector, broadcast this context back to each local feature vector, and blend the two via depthwise convolution. This technique guarantees that each convolutional layer has access to the global information in addition to the local features. Empirically, we observe that this squeeze-and-excitation technique introduces the most reduction on the WER, 2\% \zhengdong{confirm} reduction on the WER on the LibriSpeech test-clean.

In addition, we also propose other design choices of the network architecture, such as replacing the CTC loss by the RNN-T loss\cite{graves2012sequence} and using the swiss-activation function\cite{ramachandran2017searching}. Each technique contributes a slight gain; they sum up and help the model reaching the state-of-the-art WER.

To address the computation cost of a CNN model, we introduce a progressive downsampling scheme on the input utterance for more aggressive downsampling. This allow us to reduce the filter size of all the convolution layers to five without significantly reducing the effective receptive field of the entire encoder. As a benefit, we reduce the length of the encoded sequence by as large as $8\times$ while maintaining the model accuracy.

Inspired by the recent works on network scaling~\cite{tan2019efficientnet}, we also allow our net to scale with the number of channels of a convolution filter, enabling us to scale up the network for lower WER at the cost of increased computation, or to significantly reduce the computation while maintaining good WER.

In summary, the main contributions of this paper are:
\begin{itemize}
    \item A CNN encoder architecture with global context that outperforms existing CNN and transformer based models in accuracy,
    \item A progressive downsampling and model scaling scheme to achieve the best accuracy and computation trade-off.
\end{itemize}



==> LaTeX/01_model.tex <==
\section{Model}
This section introduces the architecture details of our network. Section~\ref{sec:model:transducer} discusses the high-level design of the network. Then Section~\ref{sec:model:encoder} introduces our convolutional encoder, the most important contribution of this paper. Later Section~\ref{sec:model:encoder_efficiency} discusses how we progressively reduce the temporal length of the input utterance in the network to reduce the computation while maintaining the accuracy. This section concludes with the discussion on model scaling. 

\subsection{End-to-end network: CNN-RNN-Transducer}
\label{sec:model:transducer}
Our network design is based on the RNN-Transducer framework \cite{graves2012sequence, rao2017exploring, he2017streaming}. The network contains three components: audio encoder on the input utterance, label encoder on the input label and a joint network to combine the two and decode. 

We directly use the label encoder and the joint network from \cite{zhang2020transformer}, but propose a new CNN based audio encoder. 

\subsection{Encoder design}
\label{sec:model:encoder}
Let the input sequence be $x^0=(x_1, \ldots, x_T)$ where $T$ is the temporal length of the sequence and $x_i \in\mathbb{R}^N$ is the $N$ dimensional features of each audio frame. The audio encoder operates on $x^0$ and outputs a sequence of encoded features $y=(y_1, \ldots, y_{T'})$ where $y_j\in\mathbb{R}^{N'}$ and $T'$ is the encoded length. Note that here $T'\ne T$ because the audio encoder reduces the length of sequence. To make it formal, let $\mathrm{AudioEncode}(\cdot)$ be the encoding function, we have
\begin{equation}
    (y_1, \ldots, y_{T'}) = \mathrm{AudioEncode}(x_1, \ldots, x_T).
\end{equation}

$y=(y_1, \ldots, y_{T'})$ will be the input to the RNN-T decoder.

We design the $\mathrm{AudioEncode}(\cdot)$ function via stacking multiple blocks of convolutions. Let $\mathrm{C}_k$ represent the $k$-th block of convolution, and let $x^k = \mathrm{C}_{k}(x^{k-1})$. We have
\begin{equation}
\begin{split}
    y = \mathrm{AudioEncode}(x) = \mathrm{C}_K\left(\mathrm{C}_{K-1}\left(\ldots \mathrm{C}_{1}(x)\right)\right)
\end{split}
\end{equation}

Each $\mathrm{C}(\cdot)$ includes five layers of convolution operations, each followed by batch normalization~\cite{goodfellow2016deep} and an activation function. It also contains the skip connection~\cite{he2016deep} as well as the squeeze-and-excitation component~\cite{hu2018squeeze}. Let $m$ represents the number of convolution layers of a block. Let $\mathrm{Conv}$ represent the 1D convolution. Let $\mathrm{SE}$ represent the squeeze-and-excitation module. Under this notation, we have

\begin{equation}
\begin{split}
&\mathrm{C}(x) = \mathrm{SE}\left(f^{m-1}\left(f'(x)\right)\right) + x,\\
&f(x)=\mathrm{Act}(\mathrm{BN}(\mathrm{Conv}(x)))
\end{split}
\end{equation} where $f^m$ means stacking $m$ layers of the function $f(\cdot)$ on the input. Inside each block, the first layer $f'$ can be different from the rest $m-1$ layers $f$ in the number of input and output convolution channels as well as the convolution stride. In addition, $\mathrm{Act}$ represents the activation function, and we've tried both ReLU and swish function~\cite{ramachandran2017searching}. For reader's convenience, we repeat the definition of the swish function here:
\begin{equation}
f(x)=x\cdot \sigma(\beta x)=\frac{x}{1+\exp{\left(-\beta x\right)}},
\end{equation}
where $\beta$ is a trainable parameter. We've observed that the swish function works slightly better than ReLU. Figure~\ref{fig:conv_block} illustrates the block.

\begin{figure}
    \centering
    \includegraphics[width=0.3\columnwidth]{LaTeX/figure/skip.pdf}
    \caption{A convolution block $C_i$ contains a number of convolutions, each followed by squeeze-and-excitation, batch normalization and activation. Skip connection is applied on the output of the final convolution layer.}
    \label{fig:conv_block}
\end{figure}

The Squeeze-and-excitation~\cite{hu2018squeeze} function $\mathrm{SE}(\cdot)$ performs global average pooling on the input $x$ and transforms it into a global channelwise weight $\theta(x)$ and element wise multiply each frame by this weight. We adopt the idea to the 1D case, to be precise,
\begin{equation}
\begin{split}
    \bar{x}&=\frac{1}{T} \sum_{t} x_t\\
    \theta(x)&=\mathrm{Sigmoid}(W_2(\mathrm{Act}(W_1\bar{x} + b_1)) + b_2) \\
    \mathrm{SE}(x)&=\theta(x)\circ x \\
\end{split}
\end{equation}
where $\circ$ means element-wise multiplication. If $x\in\mathbb{R}^d$, we have $W_1\in\mathbb{R}^{d\times d/8}$, and $W_2\in\mathbb{R}^{d/8 \times d}$. Note that $\mathrm{Sigmoid}(\cdot)$ maps its input to $(0, 1)$.

Figure~\ref{fig:squeeze_and_excitation} illustrates the squeeze-and-excitation function.
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{LaTeX/figure/SqueezeAndExcitation.pdf}
    \caption{1D Squeeze-and-excitation module. The input first goes through a convolution layer followed by batch normalization and activation. Then average pooling is applied to condense the conv result into a 1D vector, which is then processed by a bottleneck structure formed by two fully connected (FC) layers with activation functions. The output goes through a Sigmoid function to be mapped to $(0, 1)$, and then tiled and applied on the conv output using pointwise multiplications.}
    \label{fig:squeeze_and_excitation}
\end{figure*}

In our final design, the network has $17$ convolution blocks $C_0, \ldots, C_{16}$. Except $C_0$ and $C_{16}$ which only have one layer of convolution each, all the other convolution blocks have $5$ layers of convolution.

\subsection{Encoder efficiency}
\label{sec:model:encoder_efficiency}
\subsubsection{Progressive downsampling} We use a convolution layer of stride two to reduce the temporal length of the signal by half. In contrast to the previous CNN models that only downsample the input signal at the first layer only, we progressively apply downsampling at three different convolution blocks layers of the network, leading to in a total reduction factor of eight on the input signal. See Figure~\ref{fig:downsampling} for an illustration. This enables significant computation reduction since the computation cost of 1D convolution scales linearly with respect to the temporal length of the input signal. This avoids loss of information at an early stage. In addition, we include a few blocks of convolutions between two consecutive downsampling layers, allocating enough network capacity to extract rich information at a scale. As a result of this careful design, we observe no loss of accuracy when we put the encoder to the RNN-T framework. Section~\ref{sec:experiments} will validate this in experiments.

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{LaTeX/figure/Downsample.pdf}
    \caption{The encoder progressive downsamples the input utterance.}
    \label{fig:downsampling}
\end{figure}

\subsubsection{Small filter size} One of the claim from previous CNN works \cite{li2019jasper,kriman2019quartznet} is that larger filter size of the convolution layers benefit the encoder. In contrary, we set the filter size of every single convolution layer in our net to as small as five, and we observe significant improvement on the WER on LibriSpeech test clean. We suspect that the cause of this conter intuitive phenomenon is the effecitve receptive field of an encoder output node; when an output node covers too long segment of the input audio, the model overfits.

To analyze this more, we follow a previous work~\cite{luo2016understanding} and plot the normalized effective receptive field of our model compared against Jasper and QuartzNet in Figure~\ref{fig:yy} before training. We choose $4\sigma$ as the effective receptive field, and observe that the effective receptive field of our model is the smallest among all. Nevertheless, each encoder output covers $2-3$ seconds of audio, which is long enough to contain the pronunciation of a few words. This empirically demonstrates that our choice of small filter size reduces the risk of overfiting; nevertheless the receptive field is big enough to extract rich information from a long enough sequence of local neighboring audio.

\subsection{Model scaling}
Except for the final convolution layer, we allow the number of input channels and the number of output channels of our model to scale linearly with respect to a hyper parameter $\alpha$. Tuning $\alpha$ linearly affects the number of parameters as well as the flops. Due to the finding about the filter size in the previous section, we do not scale the filter size. This is different from EfficientNet which scales more than one design factors together.

Table \ref{tab:xx} summarizes the architecture details of our network. 

\begin{table}[!tb]
    \centering
    \begin{tabular}{ccccc}
        \hline
         Block ID & \makecell{\# Conv \\ Layers} & \makecell{\#Output \\channels} & \makecell{Filter \\ size} & other \\ \hline\hline
         $C_0$ & 1 & 256 & 5 & No residual \\ \hline
         $C_1$-$C_{10}$ & 5 & 256 & 5 & stride of $C_4, C_7$ is $2$\\ \hline
         $C_{11}$-$C_{29}$ & 5 & 512 & 5 & stride of $C_{11}$ is $2$ \\ \hline
         $C_{30}$ & 1 & 640 & 5 & dilation is $2$\\ \hline
    \end{tabular}
    \caption{Configuration of the network}
    \label{tab:table}
\end{table}


% \section{Relationship with the previous works}

% CNN models in speech
% Our work is inspired many previous work on using the CNN 

% ASR models

% CNN models in vision(weihan)

% \paragraph{CNN models in speech}

% Group 2: 


==> LaTeX/02_exp.tex <==
\section{Experiment}  
We conduct experiments on the Librispeech \cite{panayotov2015librispeech} dataset which consists of 970 hours of labeled speech and an additional text only corpus for language model training. We extracted 80 dimensional filterbanks features computed using a 25ms window with a stride of 10ms. 
We optimize the network using Adam\cite{adam} and a peak learning rate of $1e-3$. In the first $2000$ steps, the learning rate has a ramp up from $1e-5$ gradually improving to $1e-3$. Variational noise is introduced to the decoder as a regularization. An $\ell_2$ regularization is also incorporated to all the trainable weights in the network. To further improve the accuracy and the generalizability of the network, we employed the SpecAug\cite{park2019specaugment} technique which randomly masked out frequencies of the input utterance for data augmentation. 

\begin{figure}
\begin{centering}
\includegraphics[width=1\columnwidth]{figure/plot_1}
\par\end{centering}
\caption{LibRispeech Testother WER v.s. Model parameters}
\end{figure}

\subsection{Result on LibriSpeech}
Table \ref{tab:libri_speech_main} showed the result of our model on LibriSpeech test-clean/test-other against a few state-of-the-art methods include: transformer transducer, Jasper, QuartzNet and XXX.

Without language model, the performance of our model already surpassed the best known CNN model even with external language model. With the language model added, our model achieves the lowest word error rate among all the existing models. This clearly demonstrated the effectiveness of our model.

\begin{table}
\begin{centering}
\begin{tabular}{c|c|cc|cc}
\hline 
\multirow{2}{*}[-0.5em]{Model} & \multirow{2}{*}[-0.5em]{\#Params(M)} & \multicolumn{2}{c|}{Without LM} & \multicolumn{2}{c}{With LM}\\ \cline{3-6}
& & \makecell{test\\ clean} & \makecell{test\\ other} & \makecell{test \\clean} & \makecell{test \\ other}\\
\hline 
\hline 
QuartzNet~\cite{kriman2019quartznet}& 19 &3.90 & 11.28 & 2.69 & 7.25\tabularnewline
Hybrid~\cite{wang2019transformer}& - & - & - & 2.26 & 4.85\tabularnewline
Transformer~\cite{zhang2020transformer} & 139 & 2.4 & 5.6 & 2.0 & 4.6\tabularnewline
Ours & 30 & \textbf{2.4} & \textbf{5.4} &  & \tabularnewline
Ours & 46 & \textbf{2.3} & \textbf{5.0} &  & \tabularnewline
Ours & 112 & \textbf{2.1} & \textbf{4.6} & \textbf{2.0} & \textbf{4.1}
\\\hline
\hline 
\end{tabular}
\par\end{centering}
\caption{Comparison of our model against other existing models. Our model achieves superior performance both with and without language models.}
\label{tab:libri_speech_main}
\end{table}

% Table 1: With SE, without SE, SE with window size (a few?)

\subsection{Effect of context size}
To validate the effectiveness of adding global context in the CNN model for speech, we performed an ablation study on how the squeeze-and-excitation module affects the WER on LibriSpeech test-clean/test-other. The original model with all squeeze-and-excitation modules removed serves as the baseline to compare with the original model. 
Note that the squeeze-and-excitation module uses the whole utterance as the context; it has the maximal temporal length of context. This motivates us to study how the temporal length of the context impacts the model performance. To reduce the context to a window smaller than the whole utterance, we replace the global average pooling operator of the squeeze-and-excitation module by a convolutional averaging operator with a kernel size that corresponds to the context window; we apply the same fully connected layers on each context vector, and impose it on the feature of each time step. In this study, we tried window size of $100$ and $200$. 

Table~\ref{tab:context_size} illustrated the result.
% Performed on top of a standard model
% Table 2

\begin{table}
\begin{centering}
\begin{tabular}{c|cc}
\hline 
Context & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
None & ? & ? \tabularnewline
256 & ? & ? \tabularnewline
512 & 2.4 & 5.2\tabularnewline
1024 & 2.3 & 5.1\tabularnewline
global & \textbf{2.3} & \textbf{4.9}\\\hline
\hline 
\end{tabular}
\par\end{centering}
\caption{Ablation study on the temporal length of the context. }
\label{tab:libri_speech_main}
\end{table}


\subsection{Depth, width, filter size and downsampling}
\textit{Depth\ \ } We can increase the model capacity by adding extra convolutional blocks that maintains the number of channels of the encoded features. This also introduces additional computations. We perform a sweeping on the number of extra convolutional layers of the baseline model, and summary the WERs on LibriSpeech test-clean/test-other in Table \ref{tab:ablation_depth}. From the table, we can clearly see the reduction on WER due to the extra capacity of the network, until when the number of layers reach $XX$ and the model saturates.
\begin{table}
\begin{centering}
\begin{tabular}{c|cc}
\hline 
\# Extra Layers & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
0 & ? & ? \tabularnewline
15 & ? & ? \tabularnewline
512 & ? & ?\tabularnewline
1024 & ? & ?\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Ablation study on the depth of the network.}
\label{tab:ablation_depth}
\end{table}


\vspace{0.1in}
\noindent \textit{Width\ \ }

\begin{table}
\begin{centering}
\begin{tabular}{c|ccc}
\hline 
$\alpha$ & \#Params(M) & \makecell{test\\ clean} & \makecell{test\\ other} \\
\hline 
\hline 
1.25 & 46 & 2.3 & 4.9 \tabularnewline
1.5 & 46 & 2.2 & 4.8 \tabularnewline
1.75 & 87 & 2.2 & 4.7\tabularnewline
2 & 112 & 2.2 & 4.6\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Ablation study on the width of the network.}
\label{tab:ablation_depth}
\end{table}

We also scale the width of the network (i.e., the number of channels) and sees how it impacts the model performance. Specifically, we take the baseline model and scale up the output number of channels of all the convolutional kernels by $\alpha, \alpha > 1$. \zhengdong{What would be the observation?}

\vspace{0.1in}
\noindent
\textit{Downsampling and filter size\ \ }
Table \ref{tab:ablation_downsampling} summarizes the flops and WER on LibriSpeech with and without progressive downsampling. For the reference model with no progressive downsampling, we use the same CNN architectur from the QuartzNet, whose filter size ranges from $11$ to $70$\zhengdong{Confirm}. For the model with progressive downsampling, we sweep the filter size in $\{5, 11, 21\}$. Table \ref{tab:ablation_downsampling} suggests that progressive downsampling introduces significant saving in the number of flops. Moreover, it actually benefits the accuracy of the model slightly. In addition, with progressive downsampling, increasing the filter size hurts the model. This suggests model overfitting.

To qualitatively understand this phenomenon, we plot the initial receptive field of each of the models at each encoder output time step using the technique from \cite{luo2016understanding}. Figure ~\ref{fig:effective_receptive_field} plots the result. Clearly we can see that an encoder output of the QuartzNet architecture effecitvely covers the entire utterance spanning tens of seconds. Our network is much more modest, but still covers a few seconds of an audio sequence to extract rich enough information.

\subsection{Large scale dataset}
Finally, we show that the proposed architecture is also effective on large scale datasets. We use a experimental setup similar to \cite{Chiu19longform}, where the training set has 200K hours of public Youtube videos with semi-supervised transcripts generated by the approach in \cite{hank}. We evaluate on two test sets: \textit{Yt-long } of 87 videos with a total of 24.12 hours and \textit{Yt-short} of 119 videos with a total duration of 24.12 hours. Both sets come with diverse and challenging acoustic environments.

% Preview source code for paragraph 0

\begin{table}
\begin{centering}
\begin{tabular}{cccc}
\hline 
Model & \#Params (M) & YT-short & YT-long\tabularnewline
\hline 
\hline 
LSTM & 192 & 9.1 & 14.8\tabularnewline
CNN & 112 & 9.0 & 14.6\tabularnewline
CNN & 178 & 8.4 & 14.4\tabularnewline
\hline 
\end{tabular}
\par\end{centering}
\caption{Comparison with previous best results on Youtube test sets}

\end{table}




==> LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


